Amortized Inference of Variational Bounds for Learning Noisy-OR

Classical approaches for approximate inference depend on cleverly designed variational distributions and bounds. Modern approaches employ amortized variational inference, which uses a neural network to approximate any posterior without leveraging the structures of the generative models. In this paper, we propose Amortized Conjugate Posterior (ACP), a hybrid approach taking advantages of both types of approaches. Specifically, we use the classical methods to derive specific forms of posterior distributions and then learn the variational parameters using amortized inference. We study the effectiveness of the proposed approach on the noisy-or model and compare to both the classical and the modern approaches for approximate inference and parameter learning. Our results show that the proposed method outperforms or are at par with other approaches.

==> change.tex <==
% !TEX root = main.tex
\section*{Changes to be made}
\begin{itemize}
\item \done{Change names of Toy-Sparse/Toy-Pattern}: \yiming{changed them to PASY(pattern synthetic dataset) and SASY(sampled synthetic dataset)}
\item \done{Cite  Yoni Halpern thesis etc}\yiming{Yiming: done. His approach is more like our AVI approach instead of ACP. They added an additional "supervised signal" to ELBO} 
\item \done{Tighten section 2.3 (when explaining the dual)}: \yiming{Yiming: Done, change the notation slightly for $\psi$ and $\psi^*$. The notations in other sections are not changed yet. If you feel the notation is fine I'll modify other sections. }
\item \done{Probably explain how the data is generated}: \yiming{Yiming: done}
\item In Document classification, is the thresholding making sense?  Perhaps comparing to prior? Perhaps using the probabilities  \yiming{Yiming: new results will be out tonight}
\item \done{No need to worry. Fig. 7: seems more dimensionality can reduce the gap between AVI and ACP?}
\item \done{Fig. 8: using binary z or using continuous z?} \yiming{Yiming: approximate posterior probabilities}
\item \todo{When do we have results in section 4.7/collaborative filtering?}
%\item section 4.8: probably write out the form of the upperbound? You probably use also the upperbound likelihood for negative observation? Probably not the KL divergence in the objective function -- technically you are doing maximum likelihood estimation with an approximate (upperbound) likelihood function
\item section 4.9 why sharing the weigths in the bottom layer? What happens if you do not share? \yiming{Yiming: experiments are running}
\item \done{Specify how many samples are used in MC sampling} \yiming{Yiming: done}
\end{itemize}
